A Dual-Helix Governance Approach Towards Reliable Agentic Artificial Intelligence for WebGIS Development

WebGIS development requires consistency, yet agentic AI often fails due to LLM context constraints, forgetting, stochasticity, instruction failure, and adaptation rigidity. We propose a dual-helix governance framework reframing these as structural problems rather than capacity deficits. Using a 3-track architecture (Knowledge, Behavior, Skills) and a persistent knowledge graph, it stabilizes execution by externalizing facts and enforcing protocols. Validation shows a governed agent successfully refactored a legacy WebGIS codebase (reducing cyclomatic complexity and improving maintainability), roughly halved trial-to-trial output variance relative to static prompting in a controlled experiment, and prevented common infodemic mapping errors in a 5-condition COVID-19 cartography ablation study. Operationalized via the open-source AgentLoom toolkit, this externalized governance provides the stability necessary for production-level geospatial engineering.

==> ready_to_submit/response_to_reviewers.tex <==
\section*{Editor comments:}

The manuscript presents a timely and relevant study at the intersection of GeoAI and WebGIS development. Both reviewers recognize the contribution of reframing reliability as a governance problem and acknowledge the technical soundness of the proposed framework. At the same time, the reviews, particularly Reviewer 2, raise substantive concerns regarding validation scope, experimental design, and presentation that must be addressed before the manuscript can be considered for publication.
The following reviewer comments were taken into consideration during the peer review process.

\subsection*{Response:}

\begin{quote}
    Dear Dr Xu,

    Thank you for recognizing our contribution and we appreciate the opportunity to revise our manuscript. We thank both reviewers for their constructive feedback. We considered the full scope of their recommendations throughout our revision and we made substantial improvements to the original manuscript. The main changes can be summarized as follows:

    \begin{itemize}
        \item Extended the validation scope through implementing a completely new case study that evaluates automatic cartographic design.
        \item The new case study was conducted in a different IDE (Cursor vs. Antigravity) and with a different LLM (gpt-5.2 vs. gemini-3.5-flash), to provide further evidence of the generalizability of the framework
        \item Provided more Knowledge Graph artifacts  
        \item Made several clarifications and improvements in the text with additional details as per the comments below
    \end{itemize}

We believe that the points raised in the review reports collectively pointed out several weaknesses in the original design of this research, and in turn, addressing them substantially improved the quality of our work. We are grateful for the reviewers for their suggestions. Below, we provide a point-to-point response to each of the comments/concerns explaining how we addressed them in the revised manuscript.

In addition, as a further validation we also hosted a workshop titled "From Prompts to Protocols: Governing Agentic AI for Reliable Geospatial Programming" at the recent UCGIS Symposium in College Park, MD on June 15 \footnote{\url{https://ucgissymposium2026.sched.com/event/2KN6G/from-prompts-to-protocols-governing-agentic-ai-for-reliable-geospatial-programming}}, where we introduced participants to the Dual-Helix framework and its AgentLoom implementation. The workshop was attended by 9 participants who gained hands-on experience in using the framework. The workshop materials are available at \url{https://github.com/Keven1894/ucgis-agentloom-2026-workshop}.

Once again, thank you for considering our manuscript for publication in Transactions in GIS.

Best regards,

Levente Juhasz, Boyuan Guan and Wencong Cui
    
\end{quote}

\section*{Reviewer 1 Comments to the Author}
 
The manuscript presents a well structured and technically sound framework addressing an important challenge in agentic AI systems for WebGIS development. The conceptual contributions and real world case study provide valuable insights for both the GeoAI and software engineering communities.
The suggested revisions primarily concern clarification and presentation rather than fundamental methodological issues.

\begin{quote}
    \subsection*{Response:}
Thank you for taking the time and effort to review our manuscript and providing us with valuable feedback.
\end{quote}

\subsubsection*{Comment \#1} The proposed framework introduces several components simultaneously, including knowledge externalization, behavioral enforcement, role separation, and the self-learning cycle. While the integrated system is demonstrated in the case study, the manuscript does not clearly isolate the individual contribution of these mechanisms. It would strengthen the paper if the authors could briefly discuss which component contributes most to reliability improvements, or clarify whether the benefits mainly arise from the combined architecture.


\begin{quote}
    \subsubsection*{Response:}
    Thank you for raising this point. While we originally focused on the overall presentation of the framework, we agree that discussing each component and their contribution to the overall framework is valuable. We addressed your comments through the addition of a new case study. In this case study, we conduct an ablation study by specifically removing the Knowledge, Behavior and Skills tracks to evaluate their contribution.

    In addition, the discussion section is also improved to provide additional thoughts to the overall efficacy of the framework.
\end{quote}

\subsubsection*{Comment \#2} The framework relies heavily on the knowledge graph substrate, yet the process of constructing and maintaining this graph is only briefly described. It would be helpful if the authors could include describing: how nodes are defined (section 2.2) and providing a small illustrative example of a node definition.

\begin{quote}
\subsubsection*{Response:}
   In the original Figures 1 and 2 we attempted to show a general overview of the KGs.  However, following your suggestion the manuscript now includes a sample of the real JSON file representing a Knowledge node in the main body (Listing~\ref{lst:node-example}). We also provide a comprehensive set of examples along with a visualization of the KG built for Case Study 2 in the Supplementary Materials~\ref{supplementary-kg-definitions}.
\end{quote}

\subsubsection*{Comment \#3}The evaluation focuses primarily on a single WebGIS refactoring task (Future Shorelines). While the example is realistic and well presented, the authors may briefly discuss how the framework would perform in other geospatial workflows, such as spatial analysis pipelines, automated cartographic design, or geospatial data processing tasks.

\begin{quote}
\subsubsection*{Response:}
    Thank you for this important suggestion. We agree that the original validation efforts were quite limited. In the revised manuscript, we present a new case study that presents a different geospatial use-case, that is, web cartography during the COVID-19 pandemic. We believe that this addition provides an additional layer of evidence to support the framework's usability. In addition, we improved the discussion section by also providing our thoughts on how the framework would perform in other geospatial workflows.
\end{quote}

\subsubsection*{Comment \#4} The controlled experiment comparing unguided, static-context, and dual-helix conditions is an important part of the paper. However, the experiment uses five trials, which the authors acknowledge as a practical compromise. It would be useful if the authors could briefly discuss the statistical robustness of the results and whether similar variance reductions are expected with larger numbers of trials or with different tasks.

\begin{quote}
\subsubsection*{Response:}
    We thank the reviewer for raising this important methodological point. We agree that the practical constraint of $n=5$ trials for the refactoring experiment limits the statistical power of standard variance-based tests. To address the robustness of these results, we have made two major revisions to the manuscript:
    
    1. Addition of Effect Size Metrics: We have updated Section~\ref{section-futureshorelines-experiment} to include Cohen’s $d$ alongside the $p$-values. While the Welch’s t-test for the refactoring task yielded $p=0.169$ due to the small sample size, the difference represents a small-to-medium effect size ($d = 0.46$). This indicates a practically important reduction in trial-to-trial variance ($\sigma = 0.36$ vs. $\sigma = 0.79$). In the context of automated software engineering, we argue that this variance reduction, transforming probabilistic LLM outputs into predictable workflows, is more valuable than merely raising the maximum potential score.
    
    2. Expanded Validation Scope: To directly answer whether these benefits generalize to different tasks, we introduced a completely new case study (Section~\ref{section-case-study-covid}: COVID-19 Web Mapping). In this highly domain-specific cartography task, the unguided LLM hit a hard capability ceiling, consistently failing to apply epidemiological mapping standards. The Dual-Helix framework in this experiment raised the performance ceiling by injecting structural domain facts, yielding a large effect size ($\epsilon^2 = 0.48$).
    
    We have synthesized these findings in the Discussion section to clarify that the framework provides generalizable robustness by acting as an operational stabilizer in structured tasks, and as a capability elevator in knowledge-constrained tasks.\end{quote}
 
\section*{Reviewer 2 Comments to the Author}
 
This paper proposes a dual-helix governance framework to improve the reliability of agentic AI for WebGIS development, and tests it on the FutureShorelines project. The idea of reframing reliability as a governance problem rather than a model-capability problem is interesting, but there are several issues that make me hesitate to fully endorse the claims.

\subsection*{Major concerns}

\subsubsection*{Comment \#1} Limited validation scope. The framework is tested on only one refactoring task and one model (gpt-5.2). The authors acknowledge this in the limitations, but I think the problem is more serious than they suggest. One task, one model – it is hard to see how this supports general claims about the framework's effectiveness. Even a simple additional task (e.g., generating a small mapping component from scratch) or another model would have made the results more convincing.

\begin{quote}
\subsubsection*{Response:}
We thank the reviewer for this critical feedback. We agree that demonstrating generalizability across multiple tasks and architectures is essential for validating the framework. To directly address this concern, we have expanded our validation scope by adding a completely new case study (Section~\ref{section-case-study-covid}: Case Study 2: COVID-19 Web Mapping), implementing the reviewer's exact suggestion to generate a mapping component from scratch.

To provide more evidence of the framework's model and platform agnosticism, this new experiment was executed using a completely different model (\texttt{gemini-3.5-flash}) operating within a different agentic IDE (Google Antigravity). The task required the agent to generate interactive cartography while structurally avoiding the epidemiological mapping pitfalls identified by \citet{mooney_mapping_2020}. 

Additionally, we have expanded the discussion on evaluation constraints. The substantial computational overhead and API costs associated with executing multi-step, autonomous agentic workflows necessitate practical compromises in trial volume for massive tasks like legacy code refactoring. However, by introducing this distinct secondary task with a different model, we empirically demonstrate that the Dual-Helix architecture is generalizable. It successfully shifts from acting as an operational stabilizer in software refactoring to a capability elevator in domain-specific cartographic design.
\end{quote}


\subsubsection*{Comment \#2} Confounding variables in the experiment. Condition C (dynamic governance) changes several things at once: dynamic prompt assembly, state accumulation, self-learning, and the knowledge graph. The result shows reduced variance, but we do not know which component actually caused it. The authors mention this as a limitation but do not run any ablation. Without that, it is unclear whether the whole framework is necessary or just one part of it.

\begin{quote}
\subsubsection*{Response:}
We thank the reviewer for this methodological critique. We agree that the FutureShorelines experiment (Case Study 1) evaluated the framework as an integrated system, making it impossible to isolate which specific component drove the variance reduction. 

To answer this question and address your concern, we designed a new 5-condition ablation study within the newly added COVID-19 Web Mapping case study (Section~\ref{section-case-study-covid}). Instead of testing the framework as a monolith, we systematically isolated the specific mechanisms by removing one structural component at a time:
\begin{itemize}
    \item \textbf{Condition C (Knowledge Ablation):} Framework without externalized domain facts.
    \item \textbf{Condition D (Behaviors Ablation):} Framework without externalized behavioral constraints.
    \item \textbf{Condition E (Skills Ablation):} Framework without externalized skills.
\end{itemize}

As detailed in the Results (Section~\ref{section-covid-results}), the ablation study showed a degradation in performance. While the Full AgentLoom framework achieved the best results, removing just the Knowledge, Behaviors or Skills caused decreased performance in cartographic reliability, trending back toward the unguided baseline condition. 

By isolating these variables, we show that removing any single track degrades cartographic reliability while the complete framework performs best, and that the ablation lets us rank the per-track contributions for this task (Skills $>$ Behaviors $>$ Knowledge). This directly answers the question of which components drive the gains. We have added this per-track analysis to the Results of Case Study 2 and the clarifying distinction between the two experiments to its introductory paragraph.
\end{quote}


\subsubsection*{Comment \#3} Statistical significance is borderline. The variance reduction gives p = 0.047 (F-test), which just crosses the 0.05 threshold. The mean difference between Condition B and C is not significant (p = 0.169). The authors argue that variance reduction is more valuable in practice, but they do not quantify what a reduction of 0.43 in standard deviation actually means for a real development workflow – for example, how many extra human interventions it would avoid. Without that, the claim feels unsupported.

\begin{quote}
\subsubsection*{Response:}
We thank the reviewer for pushing us to ground this claim in practical engineering metrics. We agree that translating the abstract statistical variance into tangible workflow is useful for the readers.

To address this, we made changes to Section~\ref{section-futureshorelines-experiment} to make it clear what this means for a real-world development workflow:

\textbf{1. The ``Rewrite vs. Review'' Threshold:} We agree with the reviewer that abstract variance reduction must be grounded in operational reality. In practical software engineering, a high-variance LLM ($\sigma=0.79$) represents an operational liability because it dictates the worst-case performance of the agent. To quantify what a reduction of 0.43 in standard deviation means for our workflow, we look at the system's operational lower bounds. Under the static baseline (Condition B: $\mu=6.45$, $\sigma=0.79$), the expected lower bound of the agent's performance routinely drops into the critical failure zone (scores dropping toward $\approx 4.8$). In a real-world workflow, a developer cannot blindly merge code from a process with a lower bound this severe; the output is mathematically likely to contain catastrophic logic failures or architectural hallucinations that require the human to execute a full, manual rewrite (a high-cost intervention). By compressing the variance by 0.43 ($\sigma=0.36$) and raising the mean ($\mu=6.73$), the Dual-Helix framework fundamentally raises the operational floor of the agent. The worst-case performance is tightly clustered around structural soundness (scores $\approx 6.0$). For a human developer, this translates directly to avoided interventions: the worst-case scenario is elevated from a complete module rewrite to a standard code review (e.g., correcting minor syntax tweaks or variable names)..

\textbf{2. Shift in Statistical Reporting:} Based on this feedback regarding borderline significance, we acknowledge that relying on $p$-values for highly constrained samples ($n=5$ in Case study 1 and $n=3$ for Case study 2) distracted from the operational impact. As a result, we have removed the F-test from the manuscript and instead reported the effect size (Cohen's $d = 0.46$ for Case Study 1 and $\epsilon^2=0.48$ for Case Study 2).

\end{quote}

\subsubsection*{Comment \#4} Unclear role of human oversight. The Agent Builder role was filled by one of the authors, which introduces potential bias. Also, the "plan-first" rule requires human approval before execution. This raises the question of how autonomous the system really is. The reliability gains might come from the human checking the work rather than from the governance framework itself. The paper should report how often the human had to intervene or correct the agent.

\begin{quote}
\subsubsection*{Response:}
We thank the reviewer for raising this point regarding the boundaries of autonomy. We agree that the previous version of the manuscript did not explicitly define the boundary between system governance and task execution to rule out human bias. To address this, we have made substantial revisions to Sections~\ref{section-dual-helix-stabilization} and~\ref{section-futureshorelines-refactor}.

\textbf{1. Clarifying the Role of the Agent Builder (Section~\ref{section-dual-helix-stabilization}):} We have revised Section~\ref{section-dual-helix-stabilization} to clarify that the Agent Builder operates strictly during the "Build Phase" (acting as a systems architect defining the Knowledge Graph nodes). We also revised Section~\ref{section-futureshorelines-refactor} to clarify the human's role during the Execution Phase of the first case study (RBNERR). Because that case study involved refactoring a production legacy system, we explicitly instituted a "plan-first" rule (see also the next point), effectively acting as an active pair-programmer and CI/CD Pull Request gate to ensure system stability.

To address the reviewer's concern that the observed reliability gains were driven entirely by this human oversight rather than the governance framework itself, we designed a second case study (Section~\ref{section-case-study-covid}). In this new COVID-19 web mapping ablation study, the agent was tasked with generating the application autonomously across independent trials without any human-in-the-loop during the execution phase. The fully governed agent outperformed the unguided baseline, suggesting that the reliability gains are structurally derived from the framework, independent of human bias.

\textbf{2. Reframing the "Plan-First" Rule (Section~\ref{section-futureshorelines-refactor}):} We have reframed this rule to align with standard Continuous Integration/Continuous Deployment (CI/CD) practices. In production software engineering, true autonomy does not mean a developer pushes 2,000+ lines of code without review. The plan-first rule acts as an automated Pull Request (PR) gate. 

\textbf{3. Reporting Human Interventions:} Per the reviewer's request, we have explicitly documented the human-agent interaction frequency in Section~\ref{section-futureshorelines-refactor}. During the FutureShorelines refactoring execution phase, the human intervened 7 times. This included rejecting the initial architectural plan (forcing the agent to output to a sandboxed directory rather than overwriting production code) and acting as a Quality Assurance (QA) tester by pasting console errors and identifying UI regressions (e.g., a missing map layer).

The reviewer correctly identifies that because the human acted as an active QA gatekeeper in this first case study, the reliability gains cannot be fully decoupled from human oversight. We acknowledge this as a limitation originating from the original design of Case Study 1. To overcome this limitation, we designed Case Study 2 (the COVID-19 ablation study in Section~\ref{section-case-study-covid}), which was executed entirely autonomously without any human-in-the-loop during the execution phase. This provides an isolated, quantitative evidence that the governance framework fundamentally drives reliability independent of human code-checking.
\end{quote}

\subsubsection*{Comment \#5}  Missing a RAG baseline. The paper criticises RAG as merely "informational", but the experiment does not include a proper RAG condition. Condition B (static long prompt) is not the same as a RAG system that retrieves relevant documents per step. Without a RAG baseline, it is hard to conclude that structural governance is better than retrieval-based information.

\begin{quote}
\subsubsection*{Response:}
We thank the reviewer for pointing this out. We completely agree that Condition B (static context) is a prompt engineering baseline and does not represent a dynamic Retrieval-Augmented Generation (RAG) system. As a result, our original phrasing unfairly criticized RAG without a proper comparative baseline.

To correct this, we have reframed our claims throughout the manuscript (specifically in Sections~\ref{section-background-evolution} and~\ref{section-discussion-structural}). We have removed any claims stating that structural governance strictly outperforms RAG. Instead, we now clearly distinguish between the two as complementary but fundamentally different paradigms. We frame RAG as a powerful informational strategy (ideal for dynamically retrieving relevant documents or API documentation), while the Dual-Helix framework is a structural strategy (designed to programmatically block execution until mandatory constraints are met). Thank you for helping us clarify this distinction and ensure our claims do not overstep our experimental design.
\end{quote}

==> sections_revised/03-framework_old.tex <==
\section{A Dual-Helix Governance Approach for WebGIS Development} \label{section-framework}

\subsection{Overview: Addressing LLM Limitations Through Governance}

Section 1.2 identified five core LLM limitations that undermine reliability in WebGIS development. We address these through a \textbf{dual-helix governance approach} combined with a \textbf{3-track architecture}. In this work, dual-helix does not refer to multiple agents or role-based task decomposition. Instead, it denotes two governance axes---knowledge externalization and behavioral enforcement---that jointly stabilize a single execution-capable agent.

The 3-track architecture directly targets each limitation. The Knowledge track addresses long-context limitations (C1) by externalizing key information to a persistent graph that does not rely on attention mechanisms; it addresses cross-session forgetting (C2) by maintaining version-controlled project memory; and it addresses adaptation rigidity (C5) through immediate, auditable knowledge updates without retraining. The Behavior track addresses instruction following failure (C4) through executable constraints that are mandatory rather than advisory. The Skills track addresses output stochasticity (C3) through validated workflows that ensure reproducible execution.

Figure \ref{fig:architecture} illustrates this architecture.

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/figure1_architecture.pdf}
\caption{Dual-helix governance architecture. The approach stabilizes agentic execution through two orthogonal axes: knowledge externalization and behavioral enforcement. These axes co-evolve during project work, creating persistent governance structure.}
\label{fig:architecture}
\end{figure}

Dual-helix describes the two governance axes (knowledge, behavior), while the \textbf{3-track architecture} is the operational decomposition that adds \textbf{skills} as the execution-stabilization layer. Together, they form a cohesive system where governance axes guide execution.

\subsection{The 3-Track Architecture}

\subsubsection{Track 1: Behaviors}

Behaviors serve as the governance layer, constraining agent actions through executable protocols rather than mere suggestions. Unlike implicit rules embedded in prompts, behaviors are documented, versioned, and enforced through the knowledge graph structure. Each behavior node contains a unique identifier, a priority level (Critical, High, or Medium) that determines enforcement strictness, a clear description of the requirement, a path to detailed documentation, and links to the skills it governs and knowledge it references.

Behaviors are explicitly retrieved and enforced prior to skill execution, serving as operational constraints. Before executing any skill, the agent retrieves all governing behaviors and validates that intended actions comply with behavioral requirements. This mechanism ensures that critical constraints---such as accessibility compliance or file size limits---cannot be accidentally ignored.

\subsubsection{Track 2: Knowledge}

The knowledge track serves as institutional memory, providing persistent, auditable domain facts that ground agent understanding in verifiable information rather than potentially incorrect training data. Table \ref{tab:knowledge-types} summarizes the three types of knowledge nodes.

\begin{table}[h]
\centering
\begin{tabular}{lll}
\toprule
\textbf{Type} & \textbf{Purpose} & \textbf{Example} \\
\midrule
Category & Organize related concepts & \texttt{gis-research:ai-gis-integration} \\
Concept & Abstract domain ideas & \texttt{knowledge:event-driven-architecture} \\
Document & Specific artifacts with content & \texttt{docs/patterns/modular-design.md} \\
\bottomrule
\end{tabular}
\caption{Knowledge node types in the 3-track architecture}
\label{tab:knowledge-types}
\end{table}

Figure \ref{fig:kg} shows the knowledge graph structure developed for the FutureShore project, illustrating how domain knowledge (geospatial concepts, coastal vulnerability) and system knowledge (validation rules, file conventions) are organized hierarchically.

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/figure3_knowledge_graph.pdf}
\caption{Knowledge graph structure for the FutureShore project. The hierarchical organization includes domain knowledge (geospatial concepts, coastal vulnerability) and system knowledge (validation rules, file conventions).}
\label{fig:kg}
\end{figure}

\subsubsection{Track 3: Skills}

Skills serve as stabilized workflows, ensuring consistent execution patterns across sessions. Each skill defines its inputs, outputs, required knowledge, and governing behaviors, creating reproducible execution patterns. When executing a skill, the agent first retrieves required knowledge nodes, then loads governing behavior constraints, executes the skill process with full context, and finally validates output against behavior requirements. This interlocking ensures that skills execute consistently, informed by relevant knowledge and constrained by appropriate protocols.

\subsection{Behavioral Enforcement}

The behavioral enforcement axis addresses stochasticity and inconsistent execution through enforceable constraints. While the knowledge track provides the \textit{what} (domain facts, patterns, workflows), behavioral enforcement provides the \textit{how} (rules that must be satisfied, priorities that must be respected, constraints that cannot be violated).

Three characteristics distinguish behavioral enforcement from conventional prompting. First, behaviors are executable rather than advisory: they determine when a task is complete, and unlike prompts, they cannot simply be ignored. Second, behaviors are priority-ordered: critical behaviors (such as accessibility compliance) override medium-priority behaviors when conflicts arise. Third, behavior compliance is auditable: it can be inspected and verified through version-controlled artifacts.

\subsection{Protecting the Dual-Helix: Context Separation as an Implementation Pattern}

Role separation (builder vs. domain expert) is employed as an implementation mechanism to prevent interference between the two governance axes during long-horizon tasks. This is not a defining component of the dual-helix; it is a protective pattern to prevent interference during long-horizon execution. This addresses the context contamination problem where LLMs conflate different responsibilities over extended interactions. Figure \ref{fig:dualrole} illustrates this separation.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{figures/figure2_dualrole.pdf}
\caption{Role separation as implementation mechanism. The Agent Builder maintains system structure while the Domain Expert executes project tasks. Explicit role switches prevent context contamination.}
\label{fig:dualrole}
\end{figure}

The Agent Builder role operates at the meta-level: it maintains knowledge graph structure, validates system integrity, creates new skills, and ensures schema compliance. It never executes domain-specific tasks. The Domain Expert role operates at the task-level: it executes project-specific work, generates code, processes data, and creates documentation. It never modifies system structure. This separation reflects an explicit design choice to externalize concerns that large language models otherwise conflate in long-running interactions.
https://www.esri.com/training/catalog/search/
\subsection{Self-Learning Mechanism}

Unlike static knowledge bases, the dual-helix approach enables agents to learn during project work by constructing and extending their own knowledge graphs. Self-learning here refers to structured knowledge acquisition and validation, rather than model parameter updates or online training. Figure \ref{fig:selflearning} illustrates this process.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.85\textwidth]{figures/figure4_selflearning.pdf}
\caption{Self-learning mechanism. As agents work on project tasks, they discover, document, link, validate, and persist new knowledge.}
\label{fig:selflearning}
\end{figure}

The learning process is auditable because knowledge graph changes are persistent artifacts, unlike transient prompting. As agents work on a project, they discover new concepts, patterns, or requirements not currently in the knowledge graph; document them as knowledge nodes with appropriate metadata; link new nodes to existing knowledge structure; validate that new nodes meet schema requirements; and persist the updated graph for future sessions. This evolution creates a project memory that persists across sessions and can be transferred to similar future projects.

\subsection{Operational Reliability}

In this paper, we use the term operational reliability to refer to an agent's ability to complete a complex, multi-step WebGIS development task without human intervention, while preserving functional correctness and architectural consistency across sessions. This encompasses three interrelated dimensions: first-try task completion (the agent produces acceptable output on the first attempt without requiring human correction), functional correctness (the output meets specified requirements and domain standards), and cross-session consistency (the agent maintains coherent behavior across multiple interactions).

The dual-helix governance approach achieves operational reliability through structured governance rather than relying solely on model capability or prompt engineering. Behaviors enforce constraints by making rule compliance mandatory rather than optional. Knowledge grounds decisions by allowing domain facts to override incorrect model assumptions. Skills ensure patterns by producing consistent outputs through validated workflows. Memory persists across sessions, preventing repeated errors. This structured approach ensures reproducible outcomes: same inputs combined with the same governance structure yield consistent outputs. Knowledge graphs are version-controllable, and behaviors and skills are explicit, auditable artifacts.

